The COS CGM Compendium V: The Dichotomy of OVI Associated with Low- and High-Metallicity Cool Gas at z < 1

We analyze the \ovi\ content and kinematics for 126 {\hi}-selected absorbers at $0.14 \lesssim z \lesssim 0.73$ for which the metallicities of their cool photoionized phase have been determined. We separate the absorbers into 100 strong {\lya} forest systems (SLFSs with $15 \la$\,{\colden}\,$< 16.2$) and 26 partial Lyman Limit systems (pLLSs with $16.2\le$\,{\colden}\,$\le 17.2$). The sample is drawn from the COS CGM Compendium (CCC) and has \ovi\ coverage in $\sn \geq 8$ {\it HST}/COS G130M/G160M QSO spectra, yielding a $2\sigma$ completeness level of {\coldenovi}$\,\geq 13.6$. The \ovi\ detection rates differ substantially between low-metallicity (LM; {\xh} $\leq -1.4$) and high-metallicity (HM; {\xh} $> -1.4$) SLFSs, with 20\% and 60\% detection rates, respectively. The \ovi\ detection frequency for the HM and LM pLLSs is, however, similar at $\sim$60\%. The SLFSs and pLLSs without detected \ovi\ are consistent with the absorbing gas being in a single phase, while those with \ovi\ trace multiphase gas. We show that the \ovi\ velocity widths and column densities have different distributions in LM and HM gas. We find a strong correlation between \ovi\ column density and metallicity. The strongest (\coldenovi$\,\ga 14$) and broadest {\ovi} absorbers are nearly always associated with HM absorbers, while weaker \ovi\ absorbers are found in both LM and HM absorbers. From comparisons with galaxy-selected and blind \ovi\ surveys, we conclude absorbers with \coldenovi$\,\ga 14$ most likely arise in the circumgalactic medium (CGM) of star-forming galaxies. Absorbers with weak \ovi\ likely trace the extended CGM or intergalactic medium (IGM), while those without \ovi\ likely originate in the IGM.

==> tab7.tex <==
\footnotesize
\addtolength{\tabcolsep}{-1pt}
\startlongtable
\begin{longrotatetable}
\begin{deluxetable}{lccccccccccc}
\tablecaption{Summary of the {\ovi} properties in Machine-readable Format\label{tab:machinereadable-ovi-properties}}
\tablehead{
\colhead{Target} & \colhead{$z_{\rm abs}$} & \colhead{$v_{\rm min}$} & \colhead{$v_{\rm max}$} & \colhead{$\langle v \rangle$} & \colhead{$\sigma_{\langle v \rangle}$} & \colhead{$\langle dv_{90} \rangle$}  & \colhead{$\sigma_{\langle dv_{90} \rangle}$} & \colhead{$\log N$} & \colhead{$\sigma^{upper}_{\log N}$} & \colhead{$\sigma^{lower}_{\log N}$} & \colhead{Detection}\\
\colhead{} & \colhead{} & \colhead{({\kms})} & \colhead{({\kms})} & \colhead{({\kms})} & \colhead{({\kms})}  & \colhead{({\kms})} & \colhead{({\kms})} & \colhead{[\cmsq]} & \colhead{[\cmsq]} & \colhead{[\cmsq]} & \colhead{Flag}\\
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)}  & \colhead{(8)}  & \colhead{(9)} & \colhead{(10)} & \colhead{(11)} & \colhead{(12)}
}
\startdata
\hline
\midrule
J000559.23+160948.9 & $0.3058$ & $-100.0$ & $40.0$ & $-52.0$ & $8.8$ & $46.9$ & $12.5$ & $13.38$ & $0.10$ & $0.08$ & $0$\\[2pt]
J000559.23+160948.9 & $0.3479$ & $-50.0$ & $20.0$ & $-19.2$ & $0.9$ & $56.7$ & $1.2$ & $13.99$ & $0.02$ & $0.02$ & $0$\\[2pt]
J000559.23+160948.9 & $0.3662$ & $-50.0$ & $50.0$ & $-0.3$ & $1.9$ & $82.5$ & $2.6$ & $14.02$ & $0.03$ & $0.03$ & $0$\\[2pt]
J004222.29-103743.8 & $0.3161$ & $-60.0$ & $70.0$ & $-4.4$ & $7.8$ & $72.7$ & $11.1$ & $13.97$ & $0.12$ & $0.09$ & $0$\\[2pt]
J004705.89+031954.9 & $0.3139$ & $-50.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.39$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J004705.89+031954.9 & $0.3143$ & $-50.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.48$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J011013.14-021952.8 & $0.2272$ & $-110.0$ & $100.0$ & $-22.5$ & $2.2$ & $123.0$ & $3.2$ & $14.48$ & $0.02$ & $0.02$ & $0$\\[2pt]
J011013.14-021952.8 & $0.5365$ & $-20.0$ & $40.0$ & $4.1$ & $4.2$ & $34.8$ & $6.0$ & $13.59$ & $0.15$ & $0.11$ & $0$\\[2pt]
J011016.25-021851.0 & $0.3991$ & $-100.0$ & $80.0$ & $-6.5$ & $3.3$ & $116.1$ & $4.6$ & $14.36$ & $0.03$ & $0.03$ & $0$\\[2pt]
J011016.25-021851.0 & $0.5354$ & $-50.0$ & $40.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.44$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J011935.69-282131.4 & $0.3483$ & $-60.0$ & $10.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.09$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J011935.69-282131.4 & $0.3487$ & $-100.0$ & $40.0$ & $-34.4$ & $3.3$ & $89.8$ & $4.7$ & $14.07$ & $0.04$ & $0.04$ & $0$\\[2pt]
J012236.76-284321.3 & $0.3650$ & $-45.0$ & $80.0$ & $18.5$ & $2.2$ & $76.4$ & $3.1$ & $13.97$ & $0.03$ & $0.03$ & $0$\\[2pt]
J015513.20-450611.9 & $0.2260$ & $-100.0$ & $120.0$ & $7.8$ & $1.9$ & $108.1$ & $2.7$ & $14.18$ & $0.02$ & $0.02$ & $0$\\[2pt]
J020157.16-113233.1 & $0.3226$ & $-50.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<12.89$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J020157.16-113233.1 & $0.3231$ & $-40.0$ & $25.0$ & $-3.4$ & $3.1$ & $52.6$ & $4.4$ & $13.27$ & $0.09$ & $0.07$ & $0$\\[2pt]
J020157.16-113233.1 & $0.3234$ & $-55.0$ & $70.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.29$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J020157.16-113233.1 & $0.3245$ & $-45.0$ & $85.0$ & $16.2$ & $1.3$ & $99.9$ & $1.8$ & $14.11$ & $0.02$ & $0.02$ & $0$\\[2pt]
J023507.38-040205.6 & $0.3225$ & $-40.0$ & $40.0$ & $-1.6$ & $2.9$ & $66.1$ & $4.1$ & $13.58$ & $0.06$ & $0.05$ & $0$\\[2pt]
J024337.66-303048.0 & $0.3037$ & $-70.0$ & $70.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.24$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J024649.86-300741.3 & $0.3123$ & $-60.0$ & $100.0$ & $25.6$ & $6.1$ & $106.2$ & $8.6$ & $14.13$ & $0.07$ & $0.06$ & $0$\\[2pt]
J024649.86-300741.3 & $0.3359$ & $-50.0$ & $70.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.44$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J035128.56-142908.0 & $0.3285$ & $-70.0$ & $100.0$ & $-0.9$ & $11.6$ & $92.3$ & $16.3$ & $13.57$ & $0.12$ & $0.10$ & $0$\\[2pt]
J035128.56-142908.0 & $0.3569$ & $-160.0$ & $120.0$ & $-23.2$ & $4.0$ & $159.5$ & $5.7$ & $14.69$ & $0.03$ & $0.03$ & $0$\\[2pt]
J035128.56-142908.0 & $0.3572$ & $0.0$ & $70.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.34$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J035128.56-142908.0 & $0.4398$ & $-100.0$ & $100.0$ & $-7.1$ & $6.0$ & $85.7$ & $8.5$ & $13.96$ & $0.05$ & $0.05$ & $0$\\[2pt]
J040148.98-054056.5 & $0.2195$ & $-50.0$ & $140.0$ & $40.8$ & $2.8$ & $134.0$ & $4.0$ & $14.53$ & $0.03$ & $0.03$ & $0$\\[2pt]
J040148.98-054056.5 & $0.3238$ & $-70.0$ & $70.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.45$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J040748.42-121136.3 & $0.1672$ & $-125.0$ & $95.0$ & $-33.8$ & $0.4$ & $149.2$ & $0.5$ & $14.63$ & $0.00$ & $0.00$ & $0$\\[2pt]
J040748.42-121136.3 & $0.3607$ & $-30.0$ & $30.0$ & $0.3$ & $2.5$ & $45.1$ & $3.5$ & $12.81$ & $0.08$ & $0.07$ & $0$\\[2pt]
J044011.90-524818.0 & $0.3279$ & $-80.0$ & $80.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.18$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J044011.90-524818.0 & $0.6150$ & $-120.0$ & $135.0$ & $6.9$ & $2.3$ & $176.7$ & $3.2$ & $14.86$ & $0.02$ & $0.02$ & $0$\\[2pt]
J044011.90-524818.0 & $0.6157$ & $-20.0$ & $80.0$ & $16.0$ & $5.3$ & $72.8$ & $7.5$ & $13.85$ & $0.09$ & $0.07$ & $0$\\[2pt]
J055224.49-640210.7 & $0.3451$ & $-25.0$ & $25.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<12.67$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J055224.49-640210.7 & $0.4461$ & $-65.0$ & $65.0$ & $-1.9$ & $3.2$ & $81.8$ & $4.5$ & $13.66$ & $0.04$ & $0.04$ & $0$\\[2pt]
J063546.49-751616.8 & $0.4175$ & $-50.0$ & $95.0$ & $18.2$ & $1.3$ & $100.9$ & $1.9$ & $14.16$ & $0.02$ & $0.02$ & $0$\\[2pt]
J063546.49-751616.8 & $0.4528$ & $-20.0$ & $100.0$ & $41.0$ & $4.1$ & $80.9$ & $5.8$ & $13.63$ & $0.06$ & $0.05$ & $0$\\[2pt]
J063546.49-751616.8 & $0.4685$ & $-40.0$ & $80.0$ & $10.1$ & $3.3$ & $81.5$ & $4.6$ & $13.69$ & $0.04$ & $0.04$ & $0$\\[2pt]
J071950.89+742757.0 & $0.3777$ & $-40.0$ & $70.0$ & $9.1$ & $3.4$ & $69.4$ & $4.8$ & $13.77$ & $0.05$ & $0.05$ & $0$\\[2pt]
J075112.30+291938.3 & $0.4318$ & $-60.0$ & $80.0$ & $13.2$ & $3.8$ & $89.7$ & $5.4$ & $13.52$ & $0.05$ & $0.04$ & $0$\\[2pt]
J075112.30+291938.3 & $0.4945$ & $-30.0$ & $50.0$ & $4.4$ & $6.2$ & $57.2$ & $8.7$ & $13.02$ & $0.14$ & $0.10$ & $0$\\[2pt]
J080908.13+461925.6 & $0.6191$ & $-90.0$ & $90.0$ & $1.5$ & $3.2$ & $92.5$ & $4.5$ & $14.74$ & $0.04$ & $0.04$ & $0$\\[2pt]
J091440.38+282330.6 & $0.2442$ & $-90.0$ & $70.0$ & $-18.3$ & $4.0$ & $107.1$ & $5.7$ & $14.42$ & $0.05$ & $0.05$ & $0$\\[2pt]
J092554.44+453544.5 & $0.3096$ & $-50.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.12$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J094331.61+053131.4 & $0.2290$ & $-50.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.50$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J100102.64+594414.2 & $0.4156$ & $-60.0$ & $25.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.05$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J100102.64+594414.2 & $0.4160$ & $-80.0$ & $125.0$ & $17.8$ & $2.0$ & $122.7$ & $2.8$ & $14.46$ & $0.02$ & $0.02$ & $0$\\[2pt]
J100535.25+013445.5 & $0.4185$ & $-60.0$ & $60.0$ & $-7.9$ & $7.7$ & $90.7$ & $10.8$ & $13.39$ & $0.11$ & $0.09$ & $0$\\[2pt]
J100535.25+013445.5 & $0.4197$ & $-40.0$ & $40.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<12.94$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J100902.06+071343.8 & $0.3372$ & $-65.0$ & $40.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.52$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J101622.60+470643.3 & $0.4322$ & $-62.0$ & $52.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.51$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J104117.16+061016.9 & $0.6544$ & $-20.0$ & $40.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.26$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J104117.16+061016.9 & $0.6551$ & $-50.0$ & $30.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.38$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J104117.16+061016.9 & $0.6554$ & $-36.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.39$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J105945.24+144143.0 & $0.4658$ & $-60.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.21$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J105945.24+144143.0 & $0.5765$ & $-60.0$ & $80.0$ & $21.6$ & $7.7$ & $95.1$ & $10.9$ & $13.91$ & $0.10$ & $0.08$ & $0$\\[2pt]
J105956.14+121151.1 & $0.3324$ & $-60.0$ & $60.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.43$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J110539.79+342534.3 & $0.2388$ & $-60.0$ & $65.0$ & $0.4$ & $1.7$ & $77.2$ & $2.4$ & $14.59$ & $0.03$ & $0.03$ & $0$\\[2pt]
J111132.20+554725.9 & $0.6175$ & $-40.0$ & $75.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.24$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J111132.20+554725.9 & $0.6827$ & $-60.0$ & $20.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.22$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J111507.65+023757.5 & $0.3692$ & $-40.0$ & $30.0$ & $-7.8$ & $3.9$ & $57.2$ & $5.5$ & $13.78$ & $0.11$ & $0.09$ & $0$\\[2pt]
J111754.23+263416.6 & $0.3520$ & $-40.0$ & $50.0$ & $6.4$ & $6.8$ & $77.7$ & $9.7$ & $13.68$ & $0.14$ & $0.11$ & $0$\\[2pt]
J111754.23+263416.6 & $0.3523$ & $-30.0$ & $60.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.37$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J111908.59+211918.0 & $0.1385$ & $-95.0$ & $95.0$ & $7.8$ & $2.6$ & $95.4$ & $3.7$ & $13.80$ & $0.02$ & $0.02$ & $0$\\[2pt]
J112553.78+591021.6 & $0.6784$ & $-65.0$ & $65.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.40$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J113457.71+255527.8 & $0.4320$ & $-60.0$ & $30.0$ & $-17.0$ & $4.9$ & $67.5$ & $6.9$ & $13.77$ & $0.10$ & $0.08$ & $0$\\[2pt]
J113457.71+255527.8 & $0.4323$ & $-40.0$ & $70.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.34$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J113910.70-135044.0 & $0.3195$ & $-75.0$ & $40.0$ & $-19.4$ & $1.8$ & $84.3$ & $2.5$ & $14.02$ & $0.03$ & $0.03$ & $0$\\[2pt]
J113956.98+654749.1 & $0.3257$ & $-75.0$ & $80.0$ & $6.5$ & $1.4$ & $84.1$ & $2.0$ & $13.97$ & $0.01$ & $0.01$ & $0$\\[2pt]
J113956.98+654749.1 & $0.5279$ & $-60.0$ & $10.0$ & $-19.6$ & $5.9$ & $49.0$ & $8.4$ & $13.08$ & $0.16$ & $0.11$ & $0$\\[2pt]
J115120.46+543733.0 & $0.2525$ & $-110.0$ & $140.0$ & $7.6$ & $1.8$ & $126.0$ & $2.5$ & $14.34$ & $0.01$ & $0.01$ & $0$\\[2pt]
J115120.46+543733.0 & $0.6886$ & $-60.0$ & $60.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.19$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J121430.55+082508.1 & $0.3247$ & $-40.0$ & $60.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.36$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J121430.55+082508.1 & $0.3838$ & $-100.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.59$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J121920.93+063838.5 & $0.2823$ & $-25.0$ & $90.0$ & $15.4$ & $3.3$ & $79.2$ & $4.7$ & $13.63$ & $0.04$ & $0.04$ & $0$\\[2pt]
J122317.79+092306.9 & $0.3795$ & $-50.0$ & $40.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.32$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J122454.44+212246.3 & $0.3784$ & $-80.0$ & $80.0$ & $1.5$ & $2.6$ & $88.5$ & $3.6$ & $14.05$ & $0.03$ & $0.03$ & $0$\\[2pt]
J122454.44+212246.3 & $0.4208$ & $-40.0$ & $20.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<12.98$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J122454.44+212246.3 & $0.4214$ & $-60.0$ & $60.0$ & $-10.4$ & $4.5$ & $67.3$ & $6.4$ & $13.75$ & $0.06$ & $0.05$ & $0$\\[2pt]
J122512.93+121835.7 & $0.3250$ & $-100.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.53$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J123304.05-003134.1 & $0.3188$ & $-160.0$ & $100.0$ & $-36.1$ & $2.3$ & $159.3$ & $3.2$ & $14.69$ & $0.02$ & $0.02$ & $0$\\[2pt]
J123335.07+475800.4 & $0.2849$ & $-60.0$ & $60.0$ & $0.3$ & $5.3$ & $54.3$ & $7.5$ & $13.93$ & $0.09$ & $0.08$ & $0$\\[2pt]
J124154.02+572107.3 & $0.2179$ & $-100.0$ & $40.0$ & $4.7$ & $1.8$ & $66.1$ & $2.6$ & $14.51$ & $0.03$ & $0.03$ & $0$\\[2pt]
J124511.26+335610.1 & $0.5876$ & $-50.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.42$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J125846.65+242739.1 & $0.2262$ & $-100.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.54$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J130429.02+311308.2 & $0.3099$ & $-11.0$ & $100.0$ & $39.1$ & $2.1$ & $86.4$ & $2.9$ & $14.30$ & $0.03$ & $0.03$ & $0$\\[2pt]
J130451.40+245445.9 & $0.2763$ & $-75.0$ & $75.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.43$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J133045.15+281321.5 & $0.2755$ & $-80.0$ & $90.0$ & $7.1$ & $3.7$ & $104.0$ & $5.3$ & $14.29$ & $0.04$ & $0.04$ & $0$\\[2pt]
J134100.78+412314.0 & $0.3488$ & $-85.0$ & $95.0$ & $-2.3$ & $1.3$ & $96.6$ & $1.8$ & $14.52$ & $0.02$ & $0.02$ & $0$\\[2pt]
J134100.78+412314.0 & $0.6208$ & $-100.0$ & $50.0$ & $-0.5$ & $3.9$ & $105.6$ & $5.6$ & $14.35$ & $0.05$ & $0.04$ & $0$\\[2pt]
J134100.78+412314.0 & $0.6214$ & $-80.0$ & $130.0$ & {\nodata} & {\nodata} & {\nodata} & {\nodata} & $14.91$ & $0.02$ & $0.02$ & $0$\\[2pt]
J134100.78+412314.0 & $0.6861$ & $-60.0$ & $150.0$ & $53.4$ & $3.5$ & $101.1$ & $4.9$ & $14.80$ & $0.07$ & $0.07$ & $0$\\[2pt]
J135726.26+043541.3 & $0.6102$ & $-40.0$ & $75.0$ & $6.5$ & $2.4$ & $79.9$ & $3.4$ & $14.41$ & $0.05$ & $0.04$ & $0$\\[2pt]
J140732.25+550725.4 & $0.2433$ & $-75.0$ & $75.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.36$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J140732.25+550725.4 & $0.2469$ & $-50.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.29$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J140923.90+261820.9 & $0.5749$ & $-50.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.05$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J140923.90+261820.9 & $0.5996$ & $-50.0$ & $40.0$ & $-8.7$ & $1.2$ & $80.2$ & $1.6$ & $13.99$ & $0.02$ & $0.02$ & $0$\\[2pt]
J140923.90+261820.9 & $0.6827$ & $-85.0$ & $85.0$ & $2.0$ & $2.1$ & $93.8$ & $3.0$ & $14.08$ & $0.02$ & $0.02$ & $0$\\[2pt]
J141038.39+230447.1 & $0.3498$ & $-20.0$ & $40.0$ & $11.2$ & $2.6$ & $45.2$ & $3.6$ & $13.83$ & $0.09$ & $0.07$ & $0$\\[2pt]
J141038.39+230447.1 & $0.3510$ & $-50.0$ & $55.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.40$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J141038.39+230447.1 & $0.5351$ & $-20.0$ & $75.0$ & $23.8$ & $4.5$ & $76.7$ & $6.4$ & $13.73$ & $0.09$ & $0.07$ & $0$\\[2pt]
J141910.20+420746.9 & $0.4256$ & $-70.0$ & $10.0$ & $-27.9$ & $5.3$ & $60.4$ & $7.5$ & $13.73$ & $0.13$ & $0.10$ & $0$\\[2pt]
J142859.03+322506.8 & $0.3823$ & $-20.0$ & $80.0$ & $23.9$ & $4.9$ & $56.7$ & $6.9$ & $13.79$ & $0.09$ & $0.08$ & $0$\\[2pt]
J143511.53+360437.2 & $0.3730$ & $-60.0$ & $60.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.46$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J143748.28-014710.7 & $0.2989$ & $-90.0$ & $55.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<12.89$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J143748.28-014710.7 & $0.6127$ & $-90.0$ & $60.0$ & $-16.3$ & $2.6$ & $113.6$ & $3.7$ & $13.89$ & $0.03$ & $0.03$ & $0$\\[2pt]
J143748.28-014710.7 & $0.6812$ & $-100.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.41$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J150030.64+551708.8 & $0.3473$ & $-75.0$ & $75.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.21$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J150030.64+551708.8 & $0.3480$ & $-80.0$ & $75.0$ & $-5.8$ & $4.0$ & $110.0$ & $5.7$ & $14.04$ & $0.05$ & $0.04$ & $0$\\[2pt]
J152424.58+095829.7 & $0.5185$ & $-70.0$ & $70.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.06$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J152424.58+095829.7 & $0.5718$ & $-55.0$ & $30.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.20$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J152424.58+095829.7 & $0.6754$ & $-70.0$ & $105.0$ & $7.4$ & $2.8$ & $133.9$ & $3.9$ & $14.16$ & $0.03$ & $0.03$ & $0$\\[2pt]
J152424.58+095829.7 & $0.7289$ & $-30.0$ & $50.0$ & $3.3$ & $4.5$ & $55.7$ & $6.3$ & $13.69$ & $0.10$ & $0.08$ & $0$\\[2pt]
J155048.29+400144.9 & $0.3126$ & $-100.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.59$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J155048.29+400144.9 & $0.4273$ & $-80.0$ & $110.0$ & $23.8$ & $4.0$ & $151.9$ & $5.7$ & $14.37$ & $0.04$ & $0.04$ & $0$\\[2pt]
J155048.29+400144.9 & $0.4920$ & $-90.0$ & $90.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.46$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J155048.29+400144.9 & $0.4926$ & $-50.0$ & $50.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.33$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J155232.54+570516.5 & $0.3660$ & $-85.0$ & $65.0$ & $18.8$ & $5.1$ & $90.9$ & $7.2$ & $14.14$ & $0.05$ & $0.05$ & $0$\\[2pt]
J155232.54+570516.5 & $0.3665$ & $-50.0$ & $55.0$ & $-5.4$ & $2.3$ & $76.4$ & $3.3$ & $14.24$ & $0.04$ & $0.04$ & $0$\\[2pt]
J155304.92+354828.6 & $0.2179$ & $-50.0$ & $40.0$ & $-7.8$ & $3.0$ & $59.6$ & $4.2$ & $13.98$ & $0.06$ & $0.06$ & $0$\\[2pt]
J155304.92+354828.6 & $0.4755$ & $-75.0$ & $75.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.54$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J161916.54+334238.4 & $0.2694$ & $-70.0$ & $70.0$ & $6.4$ & $10.9$ & $75.3$ & $15.4$ & $13.86$ & $0.16$ & $0.11$ & $0$\\[2pt]
J161916.54+334238.4 & $0.4423$ & $-75.0$ & $100.0$ & $999.0$ & $999.0$ & $999.0$ & $999.0$ & $<13.13$ & {\nodata} & {\nodata} & $-1$\\[2pt]
J163201.12+373749.9 & $0.2740$ & $-60.0$ & $25.0$ & $0.1$ & $2.3$ & $54.4$ & $3.2$ & $13.94$ & $0.04$ & $0.04$ & $0$\\[2pt]
J163201.12+373749.9 & $0.4177$ & $-60.0$ & $65.0$ & $7.5$ & $2.3$ & $93.0$ & $3.3$ & $13.72$ & $0.03$ & $0.03$ & $0$\\[2pt]
J225738.20+134045.4 & $0.4989$ & $-40.0$ & $80.0$ & $24.8$ & $6.9$ & $92.4$ & $9.7$ & $14.29$ & $0.11$ & $0.09$ & $0$\\[2pt]
\enddata
\tablecomments{(1) J--Name of the background quasar; (2) Redshift of the absorber; (3) Start velocity of the integration range; (4) End velocity of the integration range; (5) Average velocity centroid of {\ovi}; (6) Velocity width of {\ovi} absorption; (7) Adopted measured column density of {\ovi} absorption; (8) Detection Flag for {\ovi} -- 0--detection, $-1$--upper limit.}
\end{deluxetable}
\end{longrotatetable}
